Sparse PCA Beyond Covariance Thresholding

In the Wishart model for sparse PCA we are given $n$ samples $Y_1,\ldots, Y_n$ drawn independently from a $d$-dimensional Gaussian distribution $N({0, Id + \beta vv^\top})$, where $\beta > 0$ and $v\in \mathbb{R}^d$ is a $k$-sparse unit vector, and we wish to recover $v$ (up to sign). We show that if $n \ge \Omega(d)$, then for every $t \ll k$ there exists an algorithm running in time $n\cdot d^{O(t)}$ that solves this problem as long as \[ \beta \gtrsim \frac{k}{\sqrt{nt}}\sqrt{\ln({2 + td/k^2})}\,. \] Prior to this work, the best polynomial time algorithm in the regime $k\approx \sqrt{d}$, called \emph{Covariance Thresholding} (proposed in [KNV15a] and analyzed in [DM14]), required $\beta \gtrsim \frac{k}{\sqrt{n}}\sqrt{\ln({2 + d/k^2})}$. For large enough constant $t$ our algorithm runs in polynomial time and has better guarantees than Covariance Thresholding. Previously known algorithms with such guarantees required quasi-polynomial time $d^{O(\log d)}$. In addition, we show that our techniques work with sparse PCA with adversarial perturbations studied in [dKNS20]. This model generalizes not only sparse PCA, but also other problems studied in prior works, including the sparse planted vector problem. As a consequence, we provide polynomial time algorithms for the sparse planted vector problem that have better guarantees than the state of the art in some regimes. Our approach also works with the Wigner model for sparse PCA. Moreover, we show that it is possible to combine our techniques with recent results on sparse PCA with symmetric heavy-tailed noise [dNNS22]. In particular, in the regime $k \approx \sqrt{d}$ we get the first polynomial time algorithm that works with symmetric heavy-tailed noise, while the algorithm from [dNNS22]. requires quasi-polynomial time in these settings.

==> content/gaussian-complexity.tex <==
\section{Facts about Gaussian and Rademacher complexities}\label{sec:gauss_rademacher}

Recall that for a bounded set $A\in \R^m$, the Gaussian complexity $\cG(A)$ is defined as
\[
\cG(A) = \E_{\bm w \sim N(0, \Id_m)}\sup_{a\in A} \sum_{i=1}^m a_i\bm w_i\,,
\]
and Rademacher complexity $\cR(A)$ is defined as
\[
\cR(A) = \E_{\bm s \sim U(\set{\pm1}^m)}\sup_{a\in A} \sum_{i=1}^m a_i\bm s_i\,,
\]
where $U(\set{\pm1}^m)$ is the uniform distribution over $\{+1,-1\}^m$.

\begin{fact}[\cite{wainwright_2019}, Proposition 5.28]\label{fact:lipschitz_transformation_complexity}
	Let $A\subset \R^m$ be a bounded set, and let 
	$\phi_1,\ldots,\phi_m : \R\to \R$ be $1$-Lipschitz functions that satisfy $\phi_i(0) = 0$ for all $i\in[m]$. 
	Denote $\phi: \R^m \to \R^m$, $\phi(x_1,\ldots, x_m) = \Paren{\phi_1(x_1),\ldots,\phi_m(x_m)}$. 
	Then
	\[
	\cG(\phi(A)) \le \cG(A) \quad \text{and} \quad
	\cR(\phi(A)) \le 2\cR(A)\,.
	\]
\end{fact}


\begin{fact}\cite{wainwright_2019}\label{fact:gaussian_rademacher_complexities_relation}
	For every bounded set $A\subset \R^m$, 
	\[
	\cR(A) \le \sqrt{\pi/2}\cdot \cG(A) \,.
	\]
\end{fact}

\begin{proof}
Let $\bm w_1,\ldots \bm w_m$ be iid standard Gaussian variables. Denote $\bm s_i = \sign(\bm w_i)$ and $\bm z_i = \abs{\bm w_i}$.
Since $\bm w_i$ are symmetric, $\bm s_i$ and $\bm z_i$ are independent. Since $\E \bm z_i = \sqrt{2/\pi}$,
\[
\cG(A) = \E \Brac{\sup_{a\in A} \sum_{i=1}^m a_i\bm w_i }= 
\E \E \Brac{\sup_{a\in A} \sum_{i=1}^m a_i \bm z_i \bm s_i \given \bm s}
\ge \sqrt{2/\pi}\E \Brac{\sup_{a\in A} \sum_{i=1}^m  a_i\bm s_i } = \cR(A)\,.
\]
\end{proof}

\begin{fact}[\cite{wainwright_2019}, Theorem 3.4]\label{fact:convex_lipshitz_function_of_rv}
	Let  $m\in \N$, $h > 0$ and let $\bm \xi_1,\ldots,\bm \xi_m$ be independent random variables such that $\forall i\in[m]$, $\Abs{\bm \xi_i} \le h$ with probability $1$. Let $L>0$ and let $f: \R^m \to \R$ be a convex $L$-Lipschitz function. Then for all $t > 0$,
	\[
	\Pr\Brac{f(\bm \xi_1,\ldots,\bm \xi_m) \ge 
		\E f(\bm \xi_1,\ldots,\bm \xi_m) + t} \le \exp\Paren{-\frac{t^2}{16\cdot L^2\cdot  h^2}}\,.
	\]
\end{fact}


\begin{lemma}\label{lem:subgaussianity_of_gradient}
	Let $m\in \N$ , $h > 0$ and let $\bm \xi_1,\ldots,\bm \xi_m$ be independent, symmetric about zero random variables such that $\forall i\in[m]$, $\Abs{\bm \xi_i} \le h$ with probability $1$. 
	Let $A\subset \R^m$ be a bounded set and denote $r_A = \sup_{a\in A}\normt{a}$. Let
	\[
	\bm S_A = \sup_{a\in A} \sum_{i=1}^m a_i\bm \xi_i\,.
	\]
	Then 
	\[
	\E\bm S_A \le 2\cdot h \cdot \cR(A) \le 3\cdot h \cdot \cG(A)\,,
	\]
	and for all $t>0$,
	\[
	\Pr\Brac{\bm S_A \ge \E\bm S_A + t} \le \exp\Paren{-\frac{t^2}{16\cdot  r_A^2 \cdot h^2}}\,.
	\]
\end{lemma}

\begin{proof}
	Let us first show the concentration bound. Consider the function $f:\R^m \to \R$ defined as $f(x) = \sup_{a\in A} \iprod{x,a}$. It is a convex function (as the supremum of convex functions), and $r_A$-Lipschitz since for all $x,y\in \R^m$,
	\[
	\iprod{x,a} - f(y) \le \iprod{x-y, a} \le \normt{a}\normt{x-y}\,,
	\]
	and if we take $\sup$ over $a\in A$, we get $f(x) - f(y) \le r_A \normt{x-y}$. The desired bound follows from \cref{fact:convex_lipshitz_function_of_rv}.
	
	Now let us bound the expectation. Denote $\bm s_i = \sign(\bm \xi_i)$ and $\bm \eta_i = \frac{1}{h} \abs{\bm \xi_i}$ so that $\bm \xi_i = h \cdot \bm s_i \cdot \bm \eta_i$. 
	Since $\bm \xi_i$ are symmetric, $\bm s_i$ and $\bm \eta_i$ are independent. We have
	\[
	\E \Brac{\sup_{a\in A} \sum_{i=1}^m a_i\bm \xi_i }= 
	\E \Brac{\E \Brac{\sup_{a\in A} \sum_{i=1}^m a_i \cdot h \cdot \bm \eta_i \bm s_i \given \bm \eta}}
	= h\cdot \E \Brac{\E \Brac{\sup_{a\in A} \sum_{i=1}^m \bm \phi_i(a_i)\cdot \bm s_i \given \bm \eta}}\,,
	\]
	where $\bm \phi_i :\R \to \R$ is defined as $\bm \phi_i(x_i) = \bm \eta_i x_i$. Since $0\leq \bm\eta_i\leq 1$ for all $i\in[m]$, we can see that $\bm \phi_1,\ldots,\bm \phi_m$ are all 1-Lipschitz. It follows from\cref{fact:lipschitz_transformation_complexity} that
	\[
	\E \Brac{\sup_{a\in A} \sum_{i=1}^m \bm \phi_i(a_i)\cdot \bm s_i \given \bm \eta} \le 2\cR(A)\,,
	\]
	and hence 
	$$\E\bm S_A\leq  2\cdot h \cdot \cR(A)\le 3\cdot h \cdot \cG(A)\,,$$ where the last inequality follows from \cref{fact:gaussian_rademacher_complexities_relation}.
\end{proof}



\begin{fact}[Sudakov's Minoration, \cite{wainwright_2019}, Theorem 5.30]\label{fact:SudakovMinoration}
	Let $A\subset \R^m$ be a bounded set. Then
	\begin{align*}
	 \sup_{\eps > 0}\frac{\eps}{2}\sqrt{\log \Abs{\cN_{\eps}(A)}} \le \cG(A) \,,
	\end{align*}
	where $\Abs{\cN_{\eps}(A)}$ is the minimal size of $\eps$-net in $A$ with respect to Euclidean distance.
\end{fact}




==> content/lemmas.tex <==
\section{Concentration of measure}\label{sec:missing_proofs}
This section contains some technical results needed for the proofs of \cref{thm:huber-loss-informal} and \cref{thm:median-algorithm-informal}.
We start by proving a concentration bound for the empirical median.


\begin{fact}[\cite{vershynin_2018}]\label{fact:epsilon-net-ball}
	Let $0 < \varepsilon < 1$. Let $\cB = \Set{v\in \R^n\suchthat \norm{v}\le 1}$.
	Then $\cB$ has an $\varepsilon$-net of size $\Paren{\frac{2+\eps}{\varepsilon}}^n$. That is,
	there exists a set $\cN_\varepsilon\subseteq \cB$ 
	of size at most $\Paren{\frac{2+\eps}{\varepsilon}}^n$ such that for any  vector 
	$u\in \cB$ there exists some $v\in \cN_\varepsilon$ such that $\norm{v-u} \le \varepsilon$.
\end{fact}


\begin{fact}[Chernoff's inequality, \cite{vershynin_2018}]\label{fact:chernoff}
	Let $\bm \zeta_1,\ldots, \bm \zeta_n$ 
	be independent Bernoulli random variables such that 
	$\Pr\Paren{\bm \zeta_i = 1} = \Pr\Paren{\bm\zeta_i = 0} = p$. 
	Then for every $\Delta > 0$,
	\[
	\Pr\Paren{\sum_{i=1}^n \bm\zeta_i \ge pn\Paren{1+ \Delta} } 
	\le 
	\Paren{ \frac{e^{-\Delta} }{ \Paren{1+\Delta}^{1+\Delta} } }^{pn}\,.
	\]
	and for every $\Delta \in (0,1)$,
	\[
	\Pr\Paren{\sum_{i=1}^n \bm\zeta_i \le pn\Paren{1- \Delta} } 
	\le 
	\Paren{ \frac{e^{-\Delta} }{ \Paren{1-\Delta}^{1-\Delta} } }^{pn}\,.
	\]
\end{fact}

\begin{fact}[Hoeffding's inequality, \cite{wainwright_2019}]\label{fact:hoeffding}
	Let $\bm z_1,\ldots, \bm z_n$
	be mutually independent random variables such that for each $i\in[n]$,
	$\bm z_i$ is supported on $\brac{-c_i, c_i}$ for some $c_i \ge 0$. 
	Then for all $t\ge 0$,
	\[
	\Pr\Paren{\Abs{\sum_{i=1}^n \Paren{\bm z_i - \E \bm z_i}} \ge t} 
	\le 2\exp\Paren{-\frac{t^2}{2\sum_{i=1}^n c_i^2}}\,.
	\]
\end{fact}
\begin{fact}[Bernstein's inequality
	\cite{wainwright_2019}]\label{fact:bernstein}
	Let $\bm z_1,\ldots, \bm z_n$
	be mutually independent random variables such that for each $i\in[n]$,
	$\bm z_i$ is supported on $\brac{-B, B}$ for some $B\ge 0$. 
	Then for all $t\ge 0$,
	\[
	\Pr\Paren{{\sum_{i=1}^n \Paren{\bm z_i - \E \bm z_i}} \ge t} 
	\le \exp\Paren{-\frac{t^2}{2\sum_{i=1}^n \E \bm z_i^2 + \frac{2Bt}{3}}}\,.
	\]
	\end{fact}

\begin{lemma}[Restate of \cref{lem:median-meta}]
	Let $\cS\subseteq [n]$ be a set of size $\gamma n$ and let $\bm z_1,\ldots, \bm z_n\in \R$ be mutually independent  random variables satisfying 
	\begin{enumerate}
		\item For all $i\in [n]$, $\bbP \Paren{\bm z_i \ge 0} = \bbP \Paren{\bm z_i \le 0}$.
		\item For some $\eps\geq 0$, for all $i\in \cS$,  $\bbP \Paren{\bm z_i\in \Brac{0,\eps}}=
		\bbP \Paren{\bm z_i \in \Brac{-\eps,0}}\geq q$.
	\end{enumerate}
	Then with probability at least $1-2\exp\Set{-\Omega\Paren{q^2\gamma^2 n}}$ the median $\bm{\hat{z}}$ satisfies
	\begin{align*}
	\Abs{\bm{\hat{z}}}\leq \eps\,.
	\end{align*}
	\begin{proof}
		Let $\bm \cZ=\Set{\bm z_1,\ldots,\bm z_n}$.
		Consider the following set:
		\begin{align*}
		\bm \cA&:=\Set{\bm z\in \bm \cZ \given \Abs{\bm z}\leq \eps}\,.
		\end{align*}
		Denote $\bm \cZ^{+} = \bm \cZ\cap  \R_{\ge 0}$, $\bm \cA^{+} = \bm \cA\cap  \R_{\ge 0}$, $\bm \cZ^{-} = \bm \cZ\cap  \R_{\le 0}$, $\bm \cA^{-} = \bm \cA\cap  \R_{\le 0}$.
		Applying Chernoff bound for $\gamma_1,\gamma_2, \gamma_3 \in (0,1)$,
		\begin{align*}
		\bbP \Paren{\Card{\bm \cZ^+}\leq \Paren{\frac{1}{2}-\gamma_1}n} & \leq \exp \Set{-\frac{\gamma_1^2\cdot n}{10}}\,,\\
		\bbP \Paren{\Card{\bm \cA}\leq (1-\gamma_2)\cdot  q\cdot  \Card{\cS}}&\leq \exp \Set{-\frac{\gamma_2^2\cdot q\cdot \Card{\cS}}{10}}\,,\\
		\bbP \Paren{\Card{\bm \cA^+}\leq \Paren{\frac{1}{2}-\gamma_3}\cdot \card{\bm \cA}
		\given \card{\bm \cA}}
		&\leq \exp \Set{-\frac{\gamma_3^2\cdot \Card{\bm \cA}}{10}}\,.
		\end{align*}
		Similar bounds hold for $\bm \cZ^-,\bm \cA^-$.
		
		Now, the median is in $\bm \cA$ if $\Card{\bm \cZ^-}+\Card{\bm \cA^+}\geq n/2$ and $\Card{\bm \cZ^+}+\Card{\bm \cA^-}\geq n/2$.
		It is enough to prove one of the two inequalities, the proof for the other is analogous. A union bound then concludes the proof.
		
		So for $\gamma_2=\gamma_3=\frac{1}{4}$, with probability at least
		 $1-\exp \Set{-\frac{\gamma_1^2\cdot n}{10}}-
		 2\exp \Set{-\Omega\Paren{q\cdot  \Card{\cS}}}$, 
		\begin{align*}
		\Card{\bm \cZ^-}+\Card{\bm \cA^+}
		\geq \Paren{\frac{1}{2}-\gamma_1}n+\frac{q\cdot  \Card{\cS}}{10}\,.
		\end{align*}
		it follows that $\Card{\bm \cZ^-}+\Card{\bm \cA^+}\geq n/2$ for
		\begin{align*}
		\gamma_1 \leq \frac{q \cdot \Card{\cS}}{10n}.
		\end{align*}
	\end{proof}
\end{lemma}

\begin{lemma}\label{lem:uniform-bound}
Let $V$ be an $m$-dimensional vector subspace of $\R^n$. 
Let $\cB \subseteq \Set{v\in V\suchthat \norm{v}\le R}$ for some $R \ge 1$ .

Let $g: \R^2 \to \R$ be a function such that for all $y\in \R$ and $\abs{x} \le R$,
$\abs{g(x,y)} \le C\abs{x}$ for some $C \ge 1$ and for any $|\Delta x|\le 1$, 
$\abs{g(x + \Delta x,y) - g(x,y)} \le K\abs{\Delta x}$ for some $K \ge 1$.

Let $\bm w\in \R^n$ be a random vector such that $\bm w_1,\ldots, \bm w_n$ are mutually independent.
For any $N\ge n$, with probability at least $1-N^{-m}$, for all $v\in \cB$,
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i,\bm w_i) - \E_{\bm w} g(v_i,\bm w_i)}}  \le 10C\sqrt{m\ln\Paren{RKN}} \cdot \norm{v} + 1/N\,.
\]
\begin{proof}
Consider some $v\in \R^n$. Since $\abs{g_i(v_i, \bm w_i)} \le C\abs{v_i}$,
 by Hoeffding's inequality,
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i, \bm w_i) - \E_{\bm w} g(v_i,\bm w_i)}}  \le  \tau C\norm{v}
\]
with probability $1-2\exp\Paren{-\tau^2/2}$.

Let $N\ge n$ and $\varepsilon = \frac{1}{2KnN}$.  Denote by $\cN_\varepsilon$ some $\varepsilon$-net in $\cB$ such that $\card{\cN_\varepsilon} \le \Paren{6\frac{R}{\varepsilon}}^m$. 
By union bound, for any $v\in \cN_\varepsilon$, 
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i, \bm w_i) - \E_{\bm w} g(v_i, \bm w_i)}}  
\le  10C \sqrt{m\ln\Paren{RKN}}\cdot \norm{v} 
\]
with probability at least $1-N^{-m}$.

Consider arbitrary $\Delta v \in V$ such that $\norm{\Delta v} \le \varepsilon$. 
For any $v\in \cN_\varepsilon$ and $w \in \R^n$,
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i + \Delta v_i,  w_i) - g(v_i, w_i)}} 
\le \sum_{i=1}^n\Abs{g(v_i + \Delta v_i,  w_i) - g(v_i,  w_i)}
\le K \sum_{i=1}^n \abs{\Delta v_i} \le \frac{1}{2N}\,.
\]
Hence 
\[
\Abs{\E_{\bm w} \sum_{i=1}^n\Paren{g(v_i + \Delta v_i, \bm w_i) - g(v_i, \bm w_i)}} 
\le \E_{\bm w} \Abs{\sum_{i=1}^n\Paren{g(v_i + \Delta v_i, \bm w_i) - g(v_i, \bm w_i)}} 
\le \frac{1}{2N}\,,
\] 
and
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i, \bm w_i) - \E_{\bm w} g(v_i, \bm w_i)} - 
	\sum_{i=1}^n\Paren{g(v_i + \Delta v_i, w_i) - \E_{\bm w} g(\Delta v_i, \bm w_i)}} \le 1/N\,.
\]

Therefore, with probability $1-N^{-m}$, for any $v\in \cB$,
\[
\Abs{\sum_{i=1}^n\Paren{g(v_i, \bm w_i) - \E_{\bm w} g(v_i,\bm w_i)}}  
\le 10C\sqrt{m\ln\Paren{RKN}} \cdot \norm{v} + 1/N\,.
\]
\end{proof}
\end{lemma}

\begin{lemma}\label{lem:random-set-equivalence}
	Let $\bm \zeta_1,\ldots,\bm \zeta_n$ be i.i.d. Bernoulli random variables such that 
	$\Pr\Paren{\bm \zeta_i = 1} = 1 - \Pr\Paren{\bm \zeta_i = 0} = m/n$ for some  integer  $m\le n$. 
	Denote $\bm\cS_1 = \Set{i\in [n]\suchthat \bm \zeta_i = 1}$. 
	Let $\bm \cS_2\subseteq [n]$ be a random set chosen uniformly from all subsets of $[n]$ of size exactly $m$.
	
	Let $P$ be an arbitrary property of subsets of $[n]$.
	If $\bm \cS_1$ satisfies $P$ with  probability at least $1-\varepsilon$ 
	(for some $0 \le \varepsilon \le 1$), 
	then $\bm \cS_2$ satisfies $P$ with probability at least $1-2\sqrt{n}\varepsilon$.
	\begin{proof}
		If $m=0$ or $m=n$, then $\bm \cS_1=\bm \cS_2$ with probability $1$. So it is enough to consider the case $0<m<n$.
		By Stirling's approximation, for any integer $k\ge 1$,
		\[
		\sqrt{2\pi k} \cdot\frac{k^k}{e^k}\le k! \le \sqrt{2\pi k} \cdot\frac{k^k}{e^{k-1/{(12k)}}} 
		\le 1.1\cdot\sqrt{2\pi k} \cdot\frac{k^k}{e^k}\,.
		\]
		Hence
		\[ 
		\Pr\Paren{\Card{\bm \cS_1} = m}=
		\binom{n}{m}\Paren{\frac{m}{n}}^{m}\Paren{\frac{n-m}{n}}^{n-m} \ge 
		\frac{\sqrt{n}}{1.1^2\cdot \sqrt{2\pi m(n-m)}}\ge 
		\frac{1}{2\sqrt{n}}\,.
		\]
		Therefore,
		\[
		\Pr\Paren{\bm\cS_2\notin P}=
		\Pr\Paren{\bm\cS_1\notin P \suchthat \Card{\bm \cS_1} = m}
		\le
	    \frac{\Pr\Paren{\bm\cS_1\notin P}}{\Pr\Paren{\Card{\bm \cS_1} = m}}\le
	    2\sqrt{n}\varepsilon\,.
		\]
	\end{proof}
\end{lemma}

\begin{fact}[Covariance estimation of Gaussian vectors, \cite{wainwright_2019}]\label{fact:gaussian-sample-covariance}
	Let $\bm x_1,\ldots,\bm x_n\in\R^d$ be iid $\bm x_i\sim N(0,\Sigma)$ for some positive definite $\Sigma\in\R^d$. Then, with probability at least $1-\delta$,
	\[
	\Norm{\frac{1}{n}\sum_{i=1}^n \bm x_i \transpose{\bm x_i} - \Sigma} 
	\le O\Paren{\sqrt{\frac{d + \log\Paren{1/\delta}}{n}} + \frac{d + \log\Paren{1/\delta}}{n}}
	\cdot \Norm{\Sigma}\,.
	\]
\end{fact}

\begin{lemma}\label{lem:gaussian-sample-covariance-sparse}
	Let $\bm x_1,\ldots,\bm x_n\in\R^d$ be iid $\bm x_i\sim N(0,\Sigma)$ 
	for some positive definite $\Sigma\in\R^d$. 
	Let $k\in[d]$.
	Then, with probability at least $1-\eps$, for any $k$-sparse unit vector $v\in \R^d$,
	\[
	\transpose{v}\Paren{\frac{1}{n}\sum_{i=1}^n \bm x_i \transpose{\bm x_i} - \Sigma}v
	\le O\Paren{\sqrt{\frac{k\log d + \log\Paren{1/\eps}}{n}} + \frac{k\log d + \log\Paren{1/\eps}}{n}}
	\cdot \Norm{\Sigma}\,.
	\]
\begin{proof}
	If $d=1$, $1-d^{-k} =0$ and the statement is true, so assume $d>1$.
	Consider some set $\cS\subseteq [d]$ of size at most $k$.
	By \cref{fact:gaussian-sample-covariance},  with probability at least $1-\delta$,
		for any $k$-sparse unit vector $v$ with support $\cS$,
	\[
	\transpose{v}\Paren{\frac{1}{n}\sum_{i=1}^n \bm x_i \transpose{\bm x_i} - \Sigma}v
	\le O\Paren{\sqrt{\frac{k + \log\Paren{1/\delta}}{n}} + \frac{k + \log\Paren{1/\delta}}{n}}
\cdot \Norm{\Sigma}\,.
\]
	Since there are at most $\exp\Paren{2k\ln d}$ subsets of $[d]$ of size at most $k$, the lemma follows from union bound with $\delta = \eps\exp\Paren{-3k\ln d}$.
\end{proof}
\end{lemma}

\begin{fact}[Chi-squared tail bounds, \cite{laurent2000}]\label{fact:chi-squared-tail-bounds}
	Let $X\sim \chi^2_m$ (that is, a squared norm of  standard $m$-dimensional Gaussian vector). Then for all $x>0$
 	\begin{align*}
	\bbP \Paren{X-m \geq 2x+2\sqrt{mx}} &\leq e^{-x}\\
	\bbP \Paren{m-X\geq 2\sqrt{xm}}&\leq e^{-x}
	\end{align*}
\end{fact}


\begin{fact}[Singular values of Gaussian matrix, \cite{wainwright_2019}]\label{fact:singular-values-gaussian}
	Let $W\sim N(0,1)^{n \times d}$, and assume $n\ge d$. Then for each $t\ge0$
	\[
	\Pr\Paren{\sigma_{\max}(W)\ge \sqrt{n}  + \sqrt{d} + \sqrt{t}} \le  \exp\Paren{-t/2}
	\]
	and
	\[
	\Pr\Paren{\sigma_{\min}(W)\le \sqrt{n}  - \sqrt{d} - \sqrt{t}} \le  \exp\Paren{-t/2}\,,
	\]
	where $\sigma_{\max}(W)$ and $\sigma_{\min}(W)$ are the largest and the smallest singular values of $W$.
\end{fact}

\begin{fact}[$k$-sparse norm of a Gaussian matrix]\label{fact:k-sparse-norm-gaussian}
	Let $W\sim N(0,1)^{n\times d}$ be a Gaussian matrix. Let $1\le k \le n$. Then for every $\delta > 0$
	with probability at least $1-\delta$,
	\[
	\max_{\substack{u\in\R^d\\ \norm{u}=1}}\;\;
	\max_{\substack{\text{$k$-sparse }v\in\R^n\\ \norm{v}=1}} \transpose{v}Wu \le
	\sqrt{d} + \sqrt{k} + \sqrt{2k\ln\Paren{\frac{en}{k}}} + \sqrt{2\ln(1/\delta)}
	\,.
	\]
	\begin{proof}
		Let $v$ be some $k$-sparse unit vector that maximizes the value, and let $S(v)$ be the set of nonzero coordinates of $v$.
		Consider some fixed (independend of $W$) unit $k$-sparse vector $x\in \R^n$ and the set $S(x)$ of nonzero coordinates of $x$. If we remove from $W$ all the rows with indices not from $S(x)$, we get an
		$k\times d$ Gaussian matrix $W_{S(x)}$. By \cref{fact:singular-values-gaussian}, norm of this matrix is bounded by $\sqrt{d}+\sqrt{k} + \sqrt{t}$
		with probability at least $\exp\Paren{-t/2}$. Number of all subsets $S\subseteq [n]$ of size $k$ is $\binom{n}{k}\le \Paren{\frac{en}{k}}^k$.
		By union bound, the probability that the
		norm of $W_{S(v)}$ is greater than $\sqrt{d}+\sqrt{k} + \sqrt{t}$ is at most
		\[
		\binom{n}{k}\cdot \exp\Paren{-t/2} \le \exp\Paren{k\ln\Paren{en/k} - t/2}\,.
		\]
		Taking $t = 2{k\ln\Paren{en/k} + 2\log(1/\delta)}$, we get the desired bound.
	\end{proof}
\end{fact}



\iffalse
\section{Background Information Theory}\label{sec:information-theory}

\begin{definition}[Kullback-Leibler Divergence]\label{def:divergence}
	Let $P,Q$ be probability measures over a set $\Omega$, and let $P$ be absolutely continuous with respect to $Q$, then the Kullback-Leibler divergence (or relative entropy) is defined as:
	\begin{align*}
	\kldiv{P}{Q} = \int_\Omega \log\Paren{\frac{dP}{dQ}}dP\,.
	\end{align*}
\end{definition}

\begin{fact}[Divergence of Gaussians]\label{fact:divergence_gaussian}
	Let $P,Q$ be univariate Gaussian distributions with mean and variance respectively $\mu_P,\sigma_P$ and $\mu_Q,\sigma_Q$,
	then
	\begin{align*}
	\kldiv{P}{Q} = \log \frac{\sigma_Q}{\sigma_P}+ \frac{\sigma_P^2+\Paren{\mu_P-\mu_Q}^2}{2\sigma_Q^2}-\frac{1}{2}\,.
	\end{align*}
\end{fact}

\begin{fact}[Divergence Chain Rule]\label{fact:divergence_chain_rule}
	Let $P(x_1,x_2)$ and $Q(x_1,x_2)$ be distributions over $\Omega^2$, then
	\begin{align*}
	\kldiv{P(x_1,x_2)}{Q(x_1,x_2)} = \kldiv{P(x_1)}{Q(x_1)} +\E_{x_1}\kldiv{P(x_2\given x_1)}{Q(x_2\given x_1)}\,.
	\end{align*}
\end{fact}

\begin{fact}[Divergence Tensorization Identity]\label{fact:divergence_tensorization}
	Given product probability distributions $P=P_1\times \ldots \times P_n$ and $Q=Q_1\times \ldots Q_n$, the Kullback-Leibler divergence satisfies the decoupling inequality
	\begin{align*}
	\kldiv{P}{Q}=\underset{i \in [n]}{\sum}\kldiv{P_i}{Q_i}\,.
	\end{align*}
\end{fact}

\begin{lemma}[Pinsker's Inequality]\label{lem:pinsker_inequality}
	For any distributions $P,Q$,
	\begin{align*}
	\Snorm{P-Q}_{TV}\leq \frac{1}{2}\kldiv{P}{Q}
	\end{align*}
\end{lemma}

\begin{lemma}[\Tnote{Le cam }]\label{lem:le_cam_inequality}
	For any distributions $P,Q$ over $\cZ$, and any function $\Psi:\cZ\rightarrow\Set{P,Q}$,
	\begin{align*}
	%\inf_{\Psi} \Set{P\Paren{\Psi(z)\neq 1} + Q\Paren{\Psi(z)\neq 2}} = 1- \Norm{P-Q}_{TV}
	\bbP \Paren{\Psi(z)=P\given z\sim Q} + \bbP \Paren{\Psi(z)=Q\given z\sim P} = 1- \Norm{P-Q}_{TV}\,.
	\end{align*}
	%where the infimum is taken over all tests 
\end{lemma}

\begin{definition}[$\delta$-Packing]\label{def:delta_packing}
	Let $\rho$ be a metric. A $\delta$-packing of a set $T$ with respect to $\rho$ is a subset $\Set{z_1,\ldots,z_M}\subseteq T$ such that $\rho(z_i-z_j) > \delta$ for all distinct $i,j\in [M]$. The $\delta$-packing number $M(\delta,T,\rho)$ is the cardinality of the largest $\delta$-packing.
\end{definition}

\begin{lemma}[$\delta$-Packing Euclidean Ball]\label{lem:packing_lower_bound}
	Let $\delta \in (0,1)$.	Denote with $B(d)$ the euclidean ball $\Set{y \in \R^d\given \norm{y} \leq 1}$. Then 
	\begin{align*}
		M(\delta, B(d), \Norm{\cdot})\geq \frac{1}{\delta^d}\,.
	\end{align*}
\end{lemma}

\begin{lemma}[Fano's Inequality]\label{lem:fano_inequality}
	Let $z$ be a random variable over $\cZ$ with distribution chosen uniformly at random among $\Set{P^1,\ldots,P^{M}}$. Suppose that for any distinct $i,j \in [M]$
	\begin{align*}
		\kldiv{P^i}{P^j}\geq q
	\end{align*}
	for some $q\geq 0$.
	Then for any function $\Psi:\cZ\rightarrow \Set{P^1,\ldots,P^{M}}$,
	\begin{align*}
		\sup_i \bbP \Paren{\Psi(z)\neq i\given z\sim P^i} \geq 1-\frac{q-\log 2}{\log (M-1)}\,.
	\end{align*}
\end{lemma}

\fi




==> content/preliminaries.tex <==
\section{Preliminaries}
\label{sec:preliminaries}


\paragraph{Notation}
We use boldface to denote random variables.
We hide absolute constant multiplicative factors using the standard notations $O(\cdot), \Omega(\cdot), \gtrsim, \lesssim$. 
Similarly, we hide multiplicative logarithmic (in the dimension $m$ of the input) factors using the notation $\tilde{O}(\cdot), \tilde{\Omega}(\cdot)$.  We use the notation
$\Normt{\cdot}$ for the Euclidean norm, $\Normf{\cdot}$ for the Frobenius norm,
$\Normi{X}=\max_{i \in[m]}\Abs{X_i}$. 
We write $\log$ for the logarithm to the base $e$. 

%We introduce here related background notions.

%We uselowercase letters to denote vectors,  capital letters to denote matrices and  callygraphic letters to denote tensors, e.g.: $\cT\in(\R^n)^{\otimes 3}$ denote a third-order tensor. 
%We also use calligraphic letters to denote sets, context will clarify ambiguities. To ease the reading we might at times deviate from this notation, this will be clear from context.
%
%\begin{definition}[Huber loss function]\label{def:huber-loss-function-copy}
%	The Huber loss penalty is defined as:
%	\begin{align}\label{eq:huber-penalty-copy}
%		f_h(t):=\begin{cases}
%			\frac{1}{2}t^2&\text{for }\abs{t}\leq h\,,\\
%			h(\abs{t}-\frac{h}{2})& \text{otherwise}.
%		\end{cases}
%	\end{align}
%	
%	For a vector $x\in \R^n$ we denote by $F_h(x):= \sum_{i\in [n]}f_h(x_i)$.
%\end{definition}
%
%The Huber loss satisfies the following inequality.
%
%\begin{lemma}\label[lemma]{lem:second-order-behavior-huber}
%	Let $h > 0$.
%	For all $t, \delta\in \R$, and all $0\le \zeta\le h$,
%	\begin{align}
%		f_h(t+\delta)-f_h(t)-f'_h(t)\cdot \delta\geq \frac{\delta^2}{2}\ind{\abs{t}\leq \zeta}\cdot \ind{\Abs{\delta}\leq h-\zeta}\,.
%	\end{align}
%\end{lemma}
%\begin{proof}
%	We have two cases:
%	
%	\begin{itemize}
%		\item  If $|t|>\zeta$ or $|\delta|>h-\zeta$, then either $\ind{\abs{t}\leq \zeta}=0$ or $
%		\ind{\Abs{\delta}\leq h-\zeta}=0$. Hence,
%		\begin{equation}
%			\ind{\abs{t}\leq \zeta}\cdot\ind{\Abs{\delta}\leq h-\zeta}=0\,.
%		\end{equation}
%		For this case, we simply use the convexity of $f_h$ to get
%		\begin{align}
%			f_h(t+\delta)-f_h(t)-f'_h(t)\cdot \delta&\geq 0\\
%			&= \frac{\delta^2}{2}\ind{\abs{t}\leq \zeta}\cdot \ind{\Abs{\delta}\leq h-\zeta}\,.
%		\end{align}
%		\item If $|t|\leq \zeta$ and $|\delta|\leq h-\zeta$, then $|t+\delta|\leq h$. In this case, we have $f_h(t+\delta)=\frac{1}{2}(t+\delta)^2$, $f_h(t)=\frac{1}{2}t^2$ and $f_h'(t)=t$. By direct inspection, we get
%		\begin{align}
%			f_h(t+\delta)-f_h(t)-f'_h(t)\cdot \delta&=\frac{1}{2}(t+\delta)^2-\frac{1}{2}t^2-t\delta=\frac{\delta^2}{2}\\
%			&=\frac{\delta^2}{2}\ind{\abs{t}\leq \zeta}\cdot \ind{\Abs{\delta}\leq h-\zeta}\,.
%		\end{align}
%	\end{itemize}
%\end{proof}


%\paragraph{Subspace distortion} We use $\distrtf{\Omega}$ to denote the \todo



%\paragraph{Tensors}
%For tensors $S,T\in (\R^n)^{\otimes 3}$ we define the operation
%\begin{align*}
%	\iprod{{S}\,, {T}} = \sum_{i,j,k\in[n]}{S}_{i,j,k}\cdot {T}_{i,j,k}\,.
%\end{align*}
%The injective norm of a tensor is defined as
%\begin{align*}
%	\Normin{{T}}:=\max_{\substack{x,y,z\in\R^n:\\\norm{x}=\norm{y}=\norm{z}=1}}\iprod{{T}, x\tensor y \tensor z}
%\end{align*}

%and its degree $t$-sum-of-squares relaxation as
%\begin{align*}
%	\Normins{{T}}{t} := \max_{\text{level-$t$ } \mu(x,y,z)} \pE \iprod{{T}, x\tensor y \tensor z} 	\quad\text{subj. to } \Snorm{x}=\Snorm{y}=\Snorm{z}=1\,,
%\end{align*}
%The corresponding dual norm is then
%\begin{align*}
%	\Normns{{T}}{t}:=\max_{\substack{A\in (\R^n)^{\otimes %3}:\\\Normins{{A}}{t}\leq 1}}\iprod{{T}, A}\,.
%\end{align*}
%We will refer to this norm as the sum-of-squares tensor nuclear norm.
 

\subsection{Sum of squares and pseudodistributions}

Let $x = (x_1, x_2, \ldots, x_n)$ be a tuple of $n$ indeterminates and let $\R[x]$ be the set of polynomials with real coefficients and indeterminates $x_1,\ldots,x_n$.
We say that a polynomial $p\in \R[x]$ is a \emph{sum-of-squares (sos)} if there are polynomials $q_1,\ldots,q_r$ such that $p=q_1^2 + \cdots + q_r^2$.

\subsection{Pseudo-distributions}

Pseudo-distributions are generalizations of probability distributions.
We can represent a discrete (i.e., finitely supported) probability distribution over $\R^n$ by its probability mass function $D\from \R^n \to \R$ such that $D \geq 0$ and $\sum_{x \in \mathrm{supp}(D)} D(x) = 1$.
Similarly, we can describe a pseudo-distribution by its mass function.
Here, we relax the constraint $D\ge 0$ and only require that $D$ passes certain low-degree non-negativity tests.

Concretely, a \emph{level-$\ell$ pseudo-distribution} is a finitely-supported function $D:\R^n \rightarrow \R$ such that $\sum_{x} D(x) = 1$ and $\sum_{x} D(x) f(x)^2 \geq 0$ for every polynomial $f$ of degree at most $\ell/2$.
(Here, the summations are over the support of $D$.)
A straightforward polynomial-interpolation argument shows that every level-$\infty$-pseudo distribution satisfies $D\ge 0$ and is thus an actual probability distribution.
We define the \emph{pseudo-expectation} of a function $f$ on $\R^d$ with respect to a pseudo-distribution $D$, denoted $\pE_{D(x)} f(x)$, as
\begin{equation}
	\pE_{D(x)} f(x) = \sum_{x} D(x) f(x) \,\mper
\end{equation}
The degree-$\ell$ moment tensor of a pseudo-distribution $D$ is the tensor $\E_{D(x)} (1,x_1, x_2,\ldots, x_n)^{\otimes \ell}$.
In particular, the moment tensor has an entry corresponding to the pseudo-expectation of all monomials of degree at most $\ell$ in $x$.
The set of all degree-$\ell$ moment tensors of probability distribution is a convex set.
Similarly, the set of all degree-$\ell$ moment tensors of degree $d$ pseudo-distributions is also convex.
Key to the algorithmic utility of pseudo-distributions is the fact that while there can be no efficient separation oracle for the convex set of all degree-$\ell$ moment tensors of an actual probability distribution, there's a separation oracle running in time $n^{O(\ell)}$ for the convex set of the degree-$\ell$ moment tensors of all level-$\ell$ pseudodistributions.

\begin{fact}[\cite{MR939596-Shor87,parrilo2000structured,MR1748764-Nesterov00,MR1846160-Lasserre01}]
	\label[fact]{fact:sos-separation-efficient}
	For any $n,\ell \in \N$, the following set has a $n^{O(\ell)}$-time weak separation oracle (in the sense of \cite{MR625550-Grotschel81}):
	\begin{equation}
		\Set{ \pE_{D(x)} (1,x_1, x_2, \ldots, x_n)^{\otimes d} \mid \text{ degree-d pseudo-distribution $D$ over $\R^n$}}\,\mper
	\end{equation}
\end{fact}
This fact, together with the equivalence of weak separation and optimization \cite{MR625550-Grotschel81} allows us to efficiently optimize over pseudo-distributions (approximately)---this algorithm is referred to as the sum-of-squares algorithm.

The \emph{level-$\ell$ sum-of-squares algorithm} optimizes over the space of all level-$\ell$ pseudo-distributions that satisfy a given set of polynomial constraints---we formally define this next.

\begin{definition}[Constrained pseudo-distributions]
	Let $D$ be a level-$\ell$ pseudo-distribution over $\R^n$.
	Let $\cA = \{f_1\ge 0, f_2\ge 0, \ldots, f_m\ge 0\}$ be a system of $m$ polynomial inequality constraints.
	We say that \emph{$D$ satisfies the system of constraints $\cA$ at degree $r$}, denoted $D \sdtstile{r}{} \cA$, if for every $S\subseteq[m]$ and every sum-of-squares polynomial $h$ with $\deg h + \sum_{i\in S} \max\set{\deg f_i,r}\leq \ell$,
	\begin{displaymath}
		\pE_{D} h \cdot \prod _{i\in S}f_i  \ge 0\,.
	\end{displaymath}
	We write $D \sdtstile{}{} \cA$ (without specifying the degree) if $D \sdtstile{0}{} \cA$ holds.
	Furthermore, we say that $D\sdtstile{r}{}\cA$ holds \emph{approximately} if the above inequalities are satisfied up to an error of $2^{-n^\ell}\cdot \norm{h}\cdot\prod_{i\in S}\norm{f_i}$, where $\norm{\cdot}$ denotes the Euclidean norm\footnote{The choice of norm is not important here because the factor $2^{-n^\ell}$ swamps the effects of choosing another norm.} of the cofficients of a polynomial in the monomial basis.
\end{definition}

We remark that if $D$ is an actual (discrete) probability distribution, then we have  $D\sdtstile{}{}\cA$ if and only if $D$ is supported on solutions to the constraints $\cA$.

We say that a system $\cA$ of polynomial constraints is \emph{explicitly bounded} if it contains a constraint of the form $\{ \|x\|^2 \leq M\}$.
The following fact is a consequence of \cref{fact:sos-separation-efficient} and \cite{MR625550-Grotschel81},

\begin{fact}[Efficient Optimization over Pseudo-distributions]
	There exists an $(n+ m)^{O(\ell)} $-time algorithm that, given any explicitly bounded and satisfiable system\footnote{Here, we assume that the bitcomplexity of the constraints in $\cA$ is $(n+m)^{O(1)}$.} $\cA$ of $m$ polynomial constraints in $n$ variables, outputs a level-$\ell$ pseudo-distribution that satisfies $\cA$ approximately. 
\end{fact}

\subsection{Sum-of-squares proofs}

Let $f_1, f_2, \ldots, f_r$ and $g$ be multivariate polynomials in $x$.
A \emph{sum-of-squares proof} that the constraints $\{f_1 \geq 0, \ldots, f_m \geq 0\}$ imply the constraint $\{g \geq 0\}$ consists of  sum-of-squares polynomials $(p_S)_{S \subseteq [m]}$ such that
\begin{equation}
	g = \sum_{S \subseteq [m]} p_S \cdot \prod_{i \in S} f_i
	\mper
\end{equation}
We say that this proof has \emph{degree $\ell$} if for every set $S \subseteq [m]$, the polynomial $p_S \prod_{i \in S} f_i$ has degree at most $\ell$.
If there is a degree $\ell$ SoS proof that $\{f_i \geq 0 \mid i \leq r\}$ implies $\{g \geq 0\}$, we write:
\begin{equation}
	\{f_i \geq 0 \mid i \leq r\} \sststile{\ell}{}\{g \geq 0\}
	\mper
\end{equation}


Sum-of-squares proofs satisfy the following inference rules.
For all polynomials $f,g\colon\R^n \to \R$ and for all functions $F\colon \R^n \to \R^m$, $G\colon \R^n \to \R^k$, $H\colon \R^{p} \to \R^n$ such that each of the coordinates of the outputs are polynomials of the inputs, we have:

\begin{align}
	&\frac{\cA \sststile{\ell}{} \{f \geq 0, g \geq 0 \} } {\cA \sststile{\ell}{} \{f + g \geq 0\}}, \frac{\cA \sststile{\ell}{} \{f \geq 0\}\,, \cA \sststile{\ell'}{} \{g \geq 0\}} {\cA \sststile{\ell+\ell'}{} \{f \cdot g \geq 0\}}\,, \tag{addition and multiplication}\\
	&\frac{\cA \sststile{\ell}{} \cB, \cB \sststile{\ell'}{} C}{\cA \sststile{\ell \cdot \ell'}{} C}\,,  \tag{transitivity}\\
	&\frac{\{F \geq 0\} \sststile{\ell}{} \{G \geq 0\}}{\{F(H) \geq 0\} \sststile{\ell \cdot \deg(H)} {} \{G(H) \geq 0\}} \tag{substitution}\mper
\end{align}

Low-degree sum-of-squares proofs are sound and complete if we take low-level pseudo-distributions as models.

Concretely, sum-of-squares proofs allow us to deduce properties of pseudo-distributions that satisfy some constraints.

\begin{fact}[Soundness]
	\label{fact:sos-soundness}
	If $D \sdtstile{r}{} \cA$ for a level-$\ell$ pseudo-distribution $D$ and there exists a sum-of-squares proof $\cA \sststile{r'}{} \cB$, then $D \sdtstile{r\cdot r'+r'}{} \cB$.
\end{fact}

If the pseudo-distribution $D$ satisfies $\cA$ only approximately, soundness continues to hold if we require an upper bound on the bit-complexity of the sum-of-squares $\cA \sststile{r'}{} B$  (number of bits required to write down the proof).

In our applications, the bit complexity of all sum of squares proofs will be $n^{O(\ell)}$ (assuming that all numbers in the input have bit complexity $n^{O(1)}$).
This bound suffices in order to argue about pseudo-distributions that satisfy polynomial constraints approximately.

The following fact shows that every property of low-level pseudo-distributions can be derived by low-degree sum-of-squares proofs.

\begin{fact}[Completeness]
	\label{fact:sos-completeness}
	Suppose $d \geq r' \geq r$ and $\cA$ is a collection of polynomial constraints with degree at most $r$, and $\cA \vdash \{ \sum_{i = 1}^n x_i^2 \leq B\}$ for some finite $B$.
	
	Let $\{g \geq 0 \}$ be a polynomial constraint.
	If every degree-$d$ pseudo-distribution that satisfies $D \sdtstile{r}{} \cA$ also satisfies $D \sdtstile{r'}{} \{g \geq 0 \}$, then for every $\epsilon > 0$, there is a sum-of-squares proof $\cA \sststile{d}{} \{g \geq - \epsilon \}$.
\end{fact}

We will repeatedly use the following SoS version of Cauchy-Schwarz inequality and its generalization, Hölder's inequality:
\begin{fact}[Sum-of-Squares Cauchy-Schwarz]
	Let $x,y \in \R^d$ be indeterminites. Then,
	\[ 
	\sststile{4}{x,y} \Set{\Paren{\sum_i x_i y_i}^2 \leq \Paren{\sum_i x_i^2} \Paren{\sum_i y_i^2}} \,.
	\]
	\label{fact:sos-cauchy-schwarz}
\end{fact} 

We will also use the following facts about triangle inequalities and spectral certificates within the SoS proof system.

\begin{lemma}\label[lemma]{lem:triangleSoS}
	There is a degree-2 sum-of-squares proof of the following weak triangle inequality:
	\begin{equation}
		2\left(\sum_{i=1}^n a_i^2\right) + 2\left(\sum_{i=1}^n b_i^2\right) - \left(\sum_{i=1}^n (a_i+b_i)^2\right) = \sum_{i=1}^n (a_i-b_i)^2\,.
	\end{equation}
\end{lemma}


\begin{fact}[Spectral Certificates] \label{fact:spectral-certificates}
	For any $m \times m$ matrix $A$, 
	\[
	\sststile{2}{u} \Set{ \iprod{u,Au} \leq \Norm{A}\cdot \Norm{u}_2^2}\mper
	\]
\end{fact}

We will also use the following results about pseudo-distributions.

\begin{fact}[Cauchy-Schwarz for Pseudo-distributions]
	Let $f,g$ be polynomials of degree at most $d$ in indeterminate $x \in \R^d$. Then, for any degree d pseudo-distribution $D$,
	$\pE_{D}[fg] \leq \sqrt{\pE_{D}[f^2]} \sqrt{\pE_{D}[g^2]}$.
	\label{fact:pseudo-expectation-cauchy-schwarz}
\end{fact} 

